Prompt-Driven Building Footprint Extraction in Aerial Images with Offset-Building Model

More accurate extraction of invisible building footprints from very-high-resolution (VHR) aerial images relies on roof segmentation and roof-to-footprint offset extraction. Existing methods based on instance segmentation suffer from poor generalization when extended to large-scale data production and fail to achieve low-cost human interaction. This prompt paradigm inspires us to design a promptable framework for roof and offset extraction, and transforms end-to-end algorithms into promptable methods. Within this framework, we propose a novel Offset-Building Model (OBM). Based on prompt prediction, we first discover a common pattern of predicting offsets and tailored Distance-NMS (DNMS) algorithms for offset optimization. To rigorously evaluate the algorithm's capabilities, we introduce a prompt-based evaluation method, where our model reduces offset errors by 16.6\% and improves roof Intersection over Union (IoU) by 10.8\% compared to other models. Leveraging the common patterns in predicting offsets, DNMS algorithms enable models to further reduce offset vector loss by 6.5\%. To further validate the generalization of models, we tested them using a newly proposed test set, Huizhou test set, with over 7,000 manually annotated instance samples. Our algorithms and dataset will be available at https://github.com/likaiucas/OBM.

==> sec/X_ack.tex <==
\section{Acknowledgements}
This research was funded by the National Key R&D Program of China under Grant number 2021YFB3900504.

==> sec/X_authors.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/author1.jpg}}]{Kai Li}\\
    has been awarded a Bachelor's Degree in Engineering, majoring in Spatial Information and Digital Technology at UESTC in 2021. 
    Now he is a PhD student at UCAS supervised by \href{http://www.aircas.cas.cn/ykjs/lrld/201909/t20190903_5375259.html}{Zhongming Zhao} and \href{https://people.ucas.ac.cn/~0010249}{Yu Meng}. 
    He also joined CityU of Hong Kong as a joint PhD student, and his supervisor is \href{https://zhaoxyai.github.io}{Xiangyu Zhao}. His research interests include remote sensing, computer vision, and machine learning.
    Email: \url{likai211@mails.ucas.ac.cn}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/author3.jpg}}]{Yupeng Deng}\\
    is a postgraduate at the Aerospace Information Research Institute, Chinese Academy of Sciences. 
    He received his Ph.D. degree at the University of Chinese Academy of Sciences, Chinese Academy of Sciences in 2023. 
    Dr. Deng specialized in remote sensing and change detection.
    He has won a number of championship titles in several international AI competitions. 
    Email: \url{dengyp@aircas.ac.cn}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/kong.png}}]{Yunlong Kong}\\
    received the B.S degree in geographic information system from Beijing Normal University, Beijing, China, in 2010, and the Ph.D. degree in signal and information processing from Institute of Remote Sensing and Digital Earth, Chinese Academy of Sciences, Beijing, China, in 2016.
    
    He is currently working with Aerospace Information Research Institute, Chinese Academy of Sciences. His research interests include remote sensing time-series analysis and spatiotemporal big data.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/diyou.png}}]{Diyou Liu}
    Diyou Liu received the Ph.D degree in Agricultural Information Technology, College of Land Science and Technology, China Agricultural University in 2021. He is currently a special research assistant at Aerospace Information Research Institute, Chinese Academy of Sciences, Beijing, China.
    
    Currently, his research focuses on the production of cartographic-level vector element data using intelligent interpretation methods from high-resolution remote sensing imagery.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/author2.jpg}}]{Jingbo Chen}\\
    received the Ph.D. degree in cartography and geographic information systems from the Institute of Remote Sensing Applications, Chinese Academy of Sciences in 2011.
    
    He is currently an associate professor with Aerospace Information Research Institute, Chinese Academy of Sciences, Beijing, China. His research interests cover intelligent remote sensing analysis, integrated application of communication, navigation and remote sensing.
    Email: \url{chenjb@aircas.ac.cn}
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/meng.png}}]\\
    Yu Meng received the Ph.D. degree in signal and information processing from the Institute of Remote Sensing Applications, Chinese Academy of Sciences in 2008. She is currently a professor with Aerospace Information Research Institute, Chinese Academy of Sciences, Beijing, China. She serves as editor board member of National remote sensing bulletin, Journal of image and graphics.

    Her research interests include intelligent interpretation of remote sensing image, remote sensing time series signal processing, big spatial-temporal data application.

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/author4.jpg}}]{Junxian Ma}\\
    graduated from Peking University in 2020, and now he is pursuing his PhD degree at the University of Chinese Academy of Sciences.
    He focuses on Image Generation and Conditional Video Generation. Email: \url{majunxian20@mails.ucas.ac.cn}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/chenhao.png}}]{Chenhao Wang}\\
    Chenhao Wang received his bachelor's degree from the University of Electronic Science and Technology of China, and is currently pursuing a Ph.D. degree at the University of Chinese Academy of Sciences. His research focuses on building extraction from remote sensing images.
\end{IEEEbiography}

   

   
